Reason out Your Layout: Evoking the Layout Master from Large Language Models for Text-to-Image Synthesis

Recent advancements in text-to-image (T2I) generative models have shown remarkable capabilities in producing diverse and imaginative visuals based on text prompts. Despite the advancement, these diffusion models sometimes struggle to translate the semantic content from the text into images entirely. While conditioning on the layout has shown to be effective in improving the compositional ability of T2I diffusion models, they typically require manual layout input. In this work, we introduce a novel approach to improving T2I diffusion models using Large Language Models (LLMs) as layout generators. Our method leverages the Chain-of-Thought prompting of LLMs to interpret text and generate spatially reasonable object layouts. The generated layout is then used to enhance the generated images' composition and spatial accuracy. Moreover, we propose an efficient adapter based on a cross-attention mechanism, which explicitly integrates the layout information into the stable diffusion models. Our experiments demonstrate significant improvements in image quality and layout accuracy, showcasing the potential of LLMs in augmenting generative image models.

==> sec/1_intro_deprecated.tex <==
\section{Introduction}
\label{sec:intro}

Recently, the field of image generation has made significant progress, such as DELL-E 3~\citep{} and Stable Diffusion (SD)~\citep{}. In particular, text-to-image models (T2I) that generate images based on textual descriptions, using autoregressive and diffusion techniques, have demonstrated impressive ability to produce images of exceptional quality.~\citep{}. Among those models, SD-based models have gained much more attention in the research community as they are open to the public. Despite several efforts to further improve the generation quality of SD-based models, generating realistic images given complex descriptions is still challenging. For example, when the text description involves multiple objects with complex spatial relationships, SD-based models perform poorly in composing those objects within an image.

% pitfall of how t2i model can generate proper image when text is complex, and what's the current solution
There are several pieces of evidence that demonstrate the poor compositionality of a model, such as incorrect attribute leakage binding, missing objects, or misinterpretation of the object relationship~\citep{2212.05032, 2304.03869}. There exist several methods to improve the compositionally of the SD-based models~\citep{2304.03869, 2212.05032, 2304.03869,gligen}. One principal solution is to manually inject the object position information into the model~\citep{gligen, controlnet}, without asking the model itself to infer the objects' layout. For example, \citet{gligen} takes the bounding box modality into consideration and proposes to finetune an adapter that can incorporate the layout information into the image latents. Specifically, it encodes the position and the description of each object into a vector and uses another attention-based module to guide the image latents formation. On the other hand, \citet{2305.13655} shows that instead of manually specifying the layout, one can generate the layout from text description by using large language models (LLMs) such as ChatGPT~\citep{}. 

% Limitation of the current solution - 1. rely on manual layout/ when generate layout from llm, the layout is lagged behind manual labels. 2. The layot injection is not explicit. when improved compositional ability, fid is lag behind vanilla sd.
While LLMs can be used to generate object layouts, the effect of prompting strategy on the generated layout is still underexplored. Moreover, we argue that the ways previous methods inject the layout information into the models are unnatural, as they either fail to utilize the spatial information explicitly (e.g., GLGIEN) or alter the generation process heavily by manipulating the image latents~\citep{} or the cross-attention score~\citep{}. Empirical studies show that the previous layout injection scheme improves compositionality by sacrificing the quality of the generated images, i.e., lower FID score ~\citep{} compared to vanilla SD-based moels.

This work aims to close the gap of FID between composition-aware and vanilla SD-based models. First, we awake the power of LLMs in generating reasonable layouts through Chain-of-Thought Prompting~\citep{}. Specifically, we investigate what kind of reasoning design started from the given caption can lead to a better layout response. Second, we propose an extremely simple yet effective adapter, which naturally inherits the guidance style from the stable diffusion model. In the proposed adapter, the layout information is injected via an attention mask. \xc{rewrite needed }


% Our methods aims to close the gap of fid between composiiton-aware sd and vanilla sd. (1. manual layout is not required -- llm generated/ 2. layout injection is more natural (adaptor design), thus does not harm the original pretrain weight in the sd model

% experiments....


